Object-Centric Instruction Augmentation for Robotic Manipulation

Humans interpret scenes by recognizing both the identities and positions of objects in their observations. For a robot to perform tasks such as \enquote{pick and place}, understanding both what the objects are and where they are located is crucial. While the former has been extensively discussed in the literature that uses the large language model to enrich the text descriptions, the latter remains underexplored. In this work, we introduce the \textit{Object-Centric Instruction Augmentation (OCI)} framework to augment highly semantic and information-dense language instruction with position cues. We utilize a Multi-modal Large Language Model (MLLM) to weave knowledge of object locations into natural language instruction, thus aiding the policy network in mastering actions for versatile manipulation. Additionally, we present a feature reuse mechanism to integrate the vision-language features from off-the-shelf pre-trained MLLM into policy networks. Through a series of simulated and real-world robotic tasks, we demonstrate that robotic manipulator imitation policies trained with our enhanced instructions outperform those relying solely on traditional language instructions.

==> 0-abstract.tex <==






%Recently a new trend has arisen to augment natural language instruction for robots to generalize on unseen tasks. These works have ignored the importance of the fact that the robot needs to know "where" is the object and in what direction to obtain them. 

==> 1-intro.tex <==

\cite{qi2017pointnet++}


==> experiment.tex <==

\begin{table}[htb]
\begin{center}
\caption{success rate.}
\label{table:1}
\begin{tabular}{|c|c|c|}
\hline   \textbf{tasks} & \textbf{r3m\_paper} & \textbf{our\_model} \\
\hline   sliding door & $\sim 85$ & $\sim 92$  \\
\hline   microwave oven & $\sim 35$ & $\sim 28$ \\
\hline   kitchen light & $\sim 70$  & $\sim 68$\\
\hline   cabinet door & $\sim 35$  & $\sim 18$\\
\hline   knob & $\sim 40$ &\sim 38 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> franka_experiment.tex <==
\begin{table*}[htbp]
\centering
\begin{tabular}{cccccccccc}
\toprule
Methods & Pretrain & Depth & Dataset 
&PickCube & StackCube & PickSingleYCB & Fill & Hang & Excavate \\
\midrule
RGB &\ding{55} &\ding{55} & -&45 & 91.3&  35.7& 42.5 & 83.2& 20.1\\
RGB &\ding{52} & \ding{55} & ImageNet&46.3 & 92& 27.6 & 61.3 & 88.4&19  \\
RGBD &\ding{55}& \ding{52}& -& 60.1 & 90.1& 28.2 & 48.8 & 85.7& 19.4 \\
\midrule
RGB MOCO &\ding{52}& \ding{55} & ImageNet&71.3 & 91.3&  40.7& 46.9 & 82.7& 14\\
RGB PixPro &\ding{52}& \ding{55}& ImageNet & \textcolor{red}{9.4} & 90.1 & 27.5 & 67.5 & 88.8&13.6  \\
RGB Pri3D &\ding{52}& \ding{55}& ScanNet& \textcolor{red}{10.7} & 90& 19.4& 57.4 & 88.4& 17\\
RGB PixDepth &\ding{52}& \ding{55} & ScanNet& 64.4 & 91.9& 31.9  & 64 & 87& 19\\
Ours &\ding{52}& \ding{55}   & ScanNet& 94.4 &92.6 &43.8 & 73.2&88.8 &21.3 \\
\bottomrule
\end{tabular}
\caption{Success rates on rigid body and soft body tasks. Our method consistently outperforms Baseline and SOTA in all six environments. All metrics are reported in percentage $(\%)$ with the best ones bolded. }
\label{table:main}
\end{table*}

